Gaussian process approach within a data-driven POD framework for fluid dynamics engineering problems

This work describes the implementation of a data-driven approach for the reduction of the complexity of parametrical partial differential equations (PDEs) employing Proper Orthogonal Decomposition (POD) and Gaussian Process Regression (GPR). This approach is applied initially to a literature case, the simulation of the stokes problems, and in the following to a real-world industrial problem, inside a shape optimization pipeline for a naval engineering problem.

==> sections/pod-gpr.tex <==

In this section we integrate the POD and GPR methods for a data-driven
probabilistic reduced order modeling framework. The general idea is to compute
the low-dimensional representation of the input snapshots through the POD, then
infer their distribution in the parameters space in order to approximate the
solution manifold.

The only required ingredients for the method are then the snapshots matrix
$\mathbf{Y} = \begin{bmatrix}\mathbf{y}_1 & \dotsc & \mathbf{y}_n\end{bmatrix}
\in \mathbb{R}^{\fulldim\times n}$ and the corresponding parameters matrix 
$\mathbf{X} = \begin{bmatrix}\mupar_1 & \dotsc & \mupar_n\end{bmatrix}
\in \mathbb{R}^{\pardim \times n}$, where $\mupar_i$ refers to the parametric
configuration of the system for the snapshots $\mathbf{y}_i$ for $i = 1,
\dotsc, n$. The parameter points are collected by randomly sampling the parameter space.
As introduced in Section~\ref{sec:pod}, we use the POD algorithm in order to
obtain the modes and reducing the snapshots dimension such that $\mathbf{\Xi}
= \begin{bmatrix}\boldsymbol{\xi}_1 & \dotsc & \boldsymbol{\xi}_n \end{bmatrix} =
\mathbf{U}^T\mathbf{Y} \in \mathbb{R}^{\reddim\times n}$, where $\mathbf{U} =
\begin{bmatrix} \chi_1 & \dotsc & \chi_\reddim\end{bmatrix}$ is the matrix whose
columns are the POD modes. Simplifying, the columns of $\mathbf{\Xi}$ are the
$\reddim$-dimensional representation of the corresponding column of the
snapshots matrix.

We can now exploit all this information by treating all the different
components of the modal coefficients as indipendent scalar outputs. Formally,
we define the $i$-th components of the $j$-th modal coefficient $\xi_j^i$, such
that $\boldsymbol{\xi}_j = \begin{bmatrix} \xi_j^1 \dotsc \xi_j^\reddim\end{bmatrix}^T$
with $i = 1, \dotsc, \reddim$ and $j= 1, \dotsc, n$.
Analyzing the components independentely by considering each components as a
scalar output we are able to construct a probabilistic response surface for
each component, then exploiting it to approximate the modal coefficients for
unseen parameters. We define $\reddim$ train ouputs $\boldsymbol{\Xi}_k =
\begin{bmatrix}\xi_1^k & \dotsc \xi_n^k \end{bmatrix}$ for $k = 1, \dotsc,
\reddim$, whereas the train and test parameters are defined $\mathbf{X}$ and
$\bar{\mathbf{X}}$, respectively.
%The prior joint Gaussian distributions result:
%\begin{equation}
%\boldsymbol{\Xi}_j | \mathbf{X} \sim \mathcal{N}(0, \mathbf{K}_{\Xtrain \Xtrain})\quad\text{for} \, j = 1, \dotsc, \reddim.
%\end{equation}
Using Eq.~\ref{eq:gpr_pred} we can approximate the outputs --- the modal
coefficient --- for any new parameters: 
\begin{equation}
    \boldsymbol{\xi}_* 
    = \begin{bmatrix}\xi_*^1 & \dotsc & \xi_*^\reddim\end{bmatrix}^T
    = \begin{bmatrix}
        {\boldsymbol{\bar{\Xi}}_1}|\bar{\mathbf{X}}, \mathbf{X}, \boldsymbol{\Xi}_1 & 
        \dotsc & 
        {\boldsymbol{\bar{\Xi}}_N}|\bar{\mathbf{X}}, \mathbf{X}, \boldsymbol{\Xi}_N
    \end{bmatrix}^T
    \in \R^\reddim,
\end{equation}
where the $\boldsymbol{\xi}_*$ indicates the test modal coefficient and
$\boldsymbol{\bar{\Xi}_k}$ for $k = 1, \dotsc, \reddim$ refer to the test outputs.
We remark that in this work a response surface is constructed for each of the
output components, treating these latter in an independent manner with
$\reddim$ different GPs.  
The POD modes are finally exploited in order to return to the high-dimensional
space and obtain the final approximation. In matrix form:
\begin{equation}
    \mathbf{y}_* = \mathbf{U}\boldsymbol{\xi}_*,
\end{equation}
where $\mathbf{y}_* \in \fullspace$ is the solution (for the test
parameter $\mathbf{\bar{X}}$). 

